Redshifted 21-cm bispectrum II: Impact of the spin temperature fluctuations and redshift space distortions on the signal from the Cosmic Dawn

We present a study of the 21-cm signal bispectrum (which quantifies the non-Gaussianity in the signal) from the Cosmic Dawn (CD). For our analysis, we have simulated the 21-cm signal using radiative transfer code GRIZZLY, while considering two types of sources (mini-QSOs and HMXBs) for Ly$\alpha$ coupling and the X-ray heating of the IGM. Using this simulated signal, we have, for the first time, estimated the CD 21-cm bispectra for all unique $k$-triangles and for a range of $k$ modes. We observe that the redshift evolution of the bispectra magnitude and sign follow a generic trend for both source models. However, the redshifts at which the bispectra magnitude reach their maximum and minimum values and show their sign reversal depends on the source model. When the Ly$\alpha$ coupling and the X-ray heating of the IGM occur simultaneously, we observe two consecutive sign reversals in the bispectra for small $k$-triangles (irrespective of the source models). One arising at the beginning of the IGM heating and the other at the end of Ly$\alpha$ coupling saturation. This feature can be used in principle to constrain the CD history and/or to identify the specific CD scenarios. We also quantify the impact of the spin temperature ($T_{\rm S}$) fluctuations on the bispectra. We find that $T_{\rm S}$ fluctuations have maximum impact on the bispectra magnitude for small $k$-triangles and at the stage when Ly$\alpha$ coupling reaches saturation. Furthermore, we are also the first to quantify the impact of redshift space distortions (RSD), on the CD bispectra. We find that the impact of RSD on the CD 21-cm bispectra is significant ($> 20\%$) and the level depends on the stages of the CD and the $k$-triangles for which the bispectra are being estimated.

==> Formulas.tex <==
\begin{equation}
   \Delta T_{\rm b}^{\rm {s,\, qlin}}(\textbf{k}) = \widehat{\delta T_{\rm b}}(z_{cos})\widehat{\eta}(z_{cos}) \big[\Delta_{\eta}^{\prime\:r}(\textbf{k})+\Delta^r_{\rho_{\HI},\eta^\prime}(\textbf{k})+\Delta^r_{\rho_{\rm H}}(\textbf{k}) \mu_{\textbf{k}}^2 \big]
   \label{Tb_rsd_modified}
\end{equation}

where, 
\begin{equation}
    \eta = 1-\frac{T_{\rm CMB}}{T_{\rm S}}
\end{equation}

\begin{align}
\Delta_{\eta}^{\prime \:r}(\textbf{k})  = 1+\Delta_{\eta}^r(\textbf{k}) 
\end{align}
and
\begin{equation}
  \Delta{^r}_{\rho_{\HI},\eta^\prime}(\textbf{k})  = \Delta{^r}_{\rho_{\HI}}(\textbf{k})\Delta_{\eta}^{\prime\:r}(\textbf{k}) 
\end{equation}
and
\begin{equation}
    \widehat{\delta T_{\rm b}}(z_{\rm cos}) = 27  \bar{x}_{\HI}(z_{\rm cos})  \Bigg( \frac{\Omega_{\rm b} h^2}{0.023} \Bigg) \Bigg( \frac{0.15}{\Omega_{\rm m} h^2} \frac{1+z_{\rm cos}}{10} \Bigg)^{1/2} {\rm mK} \, ,
    \label{eq:tb_average}
\end{equation}

\begin{multline}
   B^{\rm {s, qlin}}(k_1,k_2,k_3) = \Big(\widehat{\delta T_{\rm b}} \widehat{\eta}\Big)^3 \Big[\Big(B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\eta}^\prime\:\Delta_{\rho_{\HI},\eta^\prime}}\\ +B^r_{\Delta_{\eta}^\prime\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\eta}^\prime}+B^r_{\Delta_{\eta}^\prime\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\HI},\eta^\prime}}+B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\HI},\eta^\prime}} \\ +B^r_{\Delta_{\eta}^\prime\:\Delta_{\eta}^\prime\:\Delta_{\rho_{\HI},\eta^\prime}}+B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\eta}^\prime}+B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\eta}^\prime\:\Delta_{\eta}^\prime}\\ +B^r_{\Delta_{\eta}^\prime\:\Delta_{\eta}^\prime\:\Delta_{\eta}^\prime}\Big)+[\overline{\mu_1^2}]^0_0\Big(B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\eta}^\prime\:\Delta_{\eta}^\prime}+B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\eta}^\prime\:\Delta_{\rho_{\HI},\eta^\prime}}\\ +B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\eta}^\prime} +B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\HI},\eta^\prime}}\Big)+[\overline{\mu_2^2}]^0_0\Big(B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\rm H}}\:\Delta_{\eta}^\prime}\\ +B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\HI},\eta^\prime}} +B^r_{\Delta_{\eta}^\prime\:\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\HI},\eta^\prime}}+B^r_{\Delta_{\eta}^\prime\:\Delta_{\rho_{\rm H}}\:\Delta_{\eta}^\prime}\Big)\\ +[\overline{\mu_3^2}]^0_0\Big( B^r_{\Delta_{\eta}^\prime\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\rm H}}}+B^r_{\Delta_{\eta}^\prime\:\Delta_{\eta}^\prime\:\Delta_{\rho_{\rm H}}}+B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\eta}^\prime\:\Delta_{\rho_{\rm H}}}\\ +B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\rm H}}}\Big) +[\overline{\mu_1^2\mu_2^2}]^0_0\Big(B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\rm H}}\:\Delta_{\eta}^\prime}+B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\HI},\eta^\prime}}\Big)\\ +[\overline{\mu_2^2\mu_3^2}]^0_0\Big(B^r_{\Delta_{\eta}^\prime\:\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\rm H}}}+B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\rm H}}}\Big) +[\overline{\mu_1^2\mu_3^2}]^0_0\Big(B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\eta}^\prime\:\Delta_{\rho_{\rm H}}}\\ +B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\rm H}}}\Big) +[\overline{\mu_1^2\mu_2^2\mu_3^2}]^0_0\Big(B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\rm H}}}\Big)\Big]
   \label{eq:b_qlin}
\end{multline}

\begin{multline}
   B^{\rm {s, qlin}}(k_1,k_2,k_3) = \Big(\widehat{\delta T_{\rm b}} \widehat{\eta}\Big)^3 \Big[\Big(B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\eta}^\prime\:\Delta_{\rho_{\HI},\eta^\prime}}\\ +B^r_{\Delta_{\eta}^\prime\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\eta}^\prime}+B^r_{\Delta_{\eta}^\prime\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\HI},\eta^\prime}}+B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\HI},\eta^\prime}} \\ +B^r_{\Delta_{\eta}^\prime\:\Delta_{\eta}^\prime\:\Delta_{\rho_{\HI},\eta^\prime}}+B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\eta}^\prime}+B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\eta}^\prime\:\Delta_{\eta}^\prime}\\ +B^r_{\Delta_{\eta}^\prime\:\Delta_{\eta}^\prime\:\Delta_{\eta}^\prime}\Big)+[\overline{\mu_1^2}]^0_0\Big(B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\eta}^\prime\:\Delta_{\eta}^\prime}+B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\eta}^\prime\:\Delta_{\rho_{\HI},\eta^\prime}}\\ +B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\eta}^\prime} +B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\HI},\eta^\prime}}\Big)+[\overline{\mu_2^2}]^0_0\Big(B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\rm H}}\:\Delta_{\eta}^\prime}\\ +B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\HI},\eta^\prime}} +B^r_{\Delta_{\eta}^\prime\:\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\HI},\eta^\prime}}+B^r_{\Delta_{\eta}^\prime\:\Delta_{\rho_{\rm H}}\:\Delta_{\eta}^\prime}\Big)\\ +[\overline{\mu_3^2}]^0_0\Big( B^r_{\Delta_{\eta}^\prime\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\rm H}}}+B^r_{\Delta_{\eta}^\prime\:\Delta_{\eta}^\prime\:\Delta_{\rho_{\rm H}}}+B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\eta}^\prime\:\Delta_{\rho_{\rm H}}}\\ +B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\rm H}}}\Big) +[\overline{\mu_1^2\mu_2^2}]^0_0\Big(B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\rm H}}\:\Delta_{\eta}^\prime}+B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\HI},\eta^\prime}}\Big)\\ +[\overline{\mu_2^2\mu_3^2}]^0_0\Big(B^r_{\Delta_{\eta}^\prime\:\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\rm H}}}+B^r_{\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\rm H}}}\Big) +[\overline{\mu_1^2\mu_3^2}]^0_0\Big(B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\eta}^\prime\:\Delta_{\rho_{\rm H}}}\\ +B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\HI},\eta^\prime}\:\Delta_{\rho_{\rm H}}}\Big) +[\overline{\mu_1^2\mu_2^2\mu_3^2}]^0_0\Big(B^r_{\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\rm H}}\:\Delta_{\rho_{\rm H}}}\Big)\Big]
   \label{eq:b_qlin}
\end{multline}


==> table.tex <==
% Example table
\begin{table}
	\centering
	\caption{This is an example table. Captions appear above each table.
	Remember to define the quantities, symbols and units used.}
	\label{tab:example_table}
	\begin{tabular}{lccr} % four columns, alignment for each
		\hline
		A & B & C & D\\
		\hline
		1 & 2 & 3 & 4\\
		2 & 4 & 6 & 8\\
		3 & 5 & 7 & 9\\
		\hline
	\end{tabular}
\end{table}

